Adversarial Robustification via Text-to-Image Diffusion Models

Adversarial robustness has been conventionally believed as a challenging property to encode for neural networks, requiring plenty of training data. In the recent paradigm of adopting off-the-shelf models, however, access to their training data is often infeasible or not practical, while most of such models are not originally trained concerning adversarial robustness. In this paper, we develop a scalable and model-agnostic solution to achieve adversarial robustness without using any data. Our intuition is to view recent text-to-image diffusion models as "adaptable" denoisers that can be optimized to specify target tasks. Based on this, we propose: (a) to initiate a denoise-and-classify pipeline that offers provable guarantees against adversarial attacks, and (b) to leverage a few synthetic reference images generated from the text-to-image model that enables novel adaptation schemes. Our experiments show that our data-free scheme applied to the pre-trained CLIP could improve the (provable) adversarial robustness of its diverse zero-shot classification derivatives (while maintaining their accuracy), significantly surpassing prior approaches that utilize the full training data. Not only for CLIP, we also demonstrate that our framework is easily applicable for robustifying other visual classifiers efficiently.

==> figures/figure-correct.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]
{figures/time_correct_factor.png}
\caption{Qualitative comparisons of denoised images on varying correct factor $k$. We perturb each input using Gaussian noise of $\sigma=0.25$, and compare the  denoised output obtained from our zero-shot denoising defined by \eqref{eq:one-step-denoising-super}.}
\label{figure:time_correct_factor}
\vspace{-0.05in}
\end{figure}

==> figures/plot-correct.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/plot-correct.png}
\caption{ImageNet accuracy (\%) on varying correction factor $k$.}
\label{figure:plot_correct_factor}
\end{figure}

==> tables/ablation-component.tex <==
\begin{table}[t]
\centering\small
\caption{
Ablation study on zero-shot adaptation schemes. Bold indicates the best and runner-up is underlined.
}\label{table:ablation_component}
\vspace{0.03in}
\resizebox{0.7\columnwidth}{!}{
\centering\small
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{}& \multicolumn{2}{c}{Adaptation} & & \multicolumn{6}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule(lr){2-3} \cmidrule{5-10}
$\sigma$& T2I & CLIP &ACR&0.0&0.25&0.5&0.75&1.0&1.25\\
\cmidrule{1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-4}\cmidrule{5-10}
\multirow{3}{*}{0.25}&\xmark&\xmark&0.277&50.8&41.8&29.6&19.2\\
&\cmark&\xmark&0.292&\underline{52.2}&\underline{43.0}&\underline{31.8}&\underline{21.4}\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{\cmark} & \cellcolor{white}{\cmark} &\textbf{0.303}&\textbf{53.4}&\textbf{44.8}&\textbf{34.2}&\textbf{21.6}&&\\
\cmidrule{1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-4}\cmidrule{5-10}
\multirow{3}{*}{0.50}&\xmark&\xmark&0.367&42.0&35.4&29.2&23.8&17.6&13.0\\
&\cmark&\xmark&0.394&\underline{44.0}&\underline{37.0}&\underline{30.8}&\textbf{25.2}&\underline{19.4}&\underline{15.2}\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{\cmark} & 
\cellcolor{white}{\cmark} &\textbf{0.409}&\textbf{46.0}&\textbf{38.8}&\textbf{32.4}&\underline{25.0}&\textbf{20.6}&\textbf{15.4}\\
\midrule
\end{tabular}}
\vspace{-0.08in}
\vspace{-0.08in}
\end{table}


==> tables/ablation-correct_factor.tex <==
\begin{table}[t]
\centering\small
\caption{
Ablation study on $k$ \eqref{eq:timestep_scale}. Bold indicates the best.}\label{table:ablation-correct-factor}
\vspace{0.03in}
\resizebox{0.7\columnwidth}{!}{
\centering\small
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{}&&&\multicolumn{6}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule{4-9}
$\sigma$&$k$&ACR&0.0&0.25&0.5&0.75&1.0&1.25\\
\cmidrule{1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule{4-9}
\multirow{3}{*}{0.25}
&0.5&0.152&36.2&23.0&14.3&\phantom{0}6.6\\
&1.0&0.229&46.0&35.6&25.2&13.4\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{1.8} &\textbf{0.277}&\textbf{50.8}&\textbf{41.8}&\textbf{29.6}&\textbf{19.2} & & \\
\midrule
\multirow{3}{*}{0.50}
&0.5&0.080&13.2&10.2&\phantom{0}6.0&\phantom{0}4.3&\phantom{0}3.4&\phantom{0}2.0\\
&1.0&0.200&28.8&22.0&16.4&11.2&\phantom{0}8.4&\phantom{0}6.0\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{1.8} &  \textbf{0.367}&\textbf{42.0}&\textbf{35.4}&\textbf{29.2}&\textbf{23.8}&\textbf{17.6}&\textbf{13.0}\\
\bottomrule
\end{tabular}
}
\vspace{-0.2in}
\end{table}


==> tables/ablation-lambda.tex <==
\begin{table}[t]
\centering\small
\caption{
Ablation study on $\lambda$ \eqref{eq:final-person-loss}. Bold indicates the best.}\label{table:ablation-lambda}
\vspace{0.03in}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{}&&&\multicolumn{6}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule{4-9}
$\sigma$&$\lambda$&ACR&0.0&0.25&0.5&0.75&1.0&1.25\\
\cmidrule{1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule{4-9}
&0.0\phantom{0}\phantom{0}&0.270&49.6&39.0&30.0&19.6\\
0.25 &0.001&0.280&50.6&40.2&30.8&20.2&&\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{0.01\phantom{0}}  &\textbf{0.292}&\textbf{52.2}&\textbf{43.0}&\textbf{31.8}&\textbf{21.4}&&\\
&0.1\phantom{0}\phantom{0}&0.290&51.8&42.8&31.2&20.6\\
\midrule
&0.0\phantom{0}\phantom{0}&0.358&38.0&32.6&27.8&22.2&18.0&14.4\\
0.50 &0.001&0.379&40.4&35.0&30.0&24.6&\textbf{20.0}&14.6\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{0.01\phantom{0}}  &\textbf{0.394}&\textbf{44.0}&\textbf{37.0}&\textbf{30.8}&\textbf{25.2}&19.4&15.2\\
&0.1\phantom{0}\phantom{0}&0.390&43.4&37.0&30.4&24.2&\textbf{20.0}&\textbf{15.4}\\
\bottomrule
\end{tabular}
}
\vspace{-0.2in}
\end{table}


==> tables/ablation-reference-size.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\centering\small
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{}&&&\multicolumn{6}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule{4-9}
$\sigma$&\textit{shot}&ACR&0.0&0.25&0.5&0.75&1.0&1.25\\
\cmidrule{1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule{4-9}
\multirow{2}{*}{0.25}&1 &0.303&53.4&\textbf{44.8}&34.2&21.6\\
&4&\cellcolor[HTML]{EFEFEF}{\textbf{0.309}}&\cellcolor[HTML]{EFEFEF}{\textbf{54.2}}&\cellcolor[HTML]{EFEFEF}{44.2}&\cellcolor[HTML]{EFEFEF}{\textbf{35.4}}&\cellcolor[HTML]{EFEFEF}{\textbf{24.8}}&\cellcolor[HTML]{EFEFEF}{}&\cellcolor[HTML]{EFEFEF}{}\\
\midrule
\multirow{2}{*}{0.5}&1&0.409&\textbf{46.0}&38.8&32.4&25.0&20.5&15.4\\
&4&\cellcolor[HTML]{EFEFEF}{\textbf{0.428}}&\cellcolor[HTML]{EFEFEF}{45.2}&\cellcolor[HTML]{EFEFEF}{\textbf{40.2}}&\cellcolor[HTML]{EFEFEF}{\textbf{34.8}}&\cellcolor[HTML]{EFEFEF}{\textbf{27.2}}&\cellcolor[HTML]{EFEFEF}{\textbf{21.6}}&\cellcolor[HTML]{EFEFEF}{\textbf{17.0}}\\
\bottomrule
\end{tabular}
}\caption{
Ablation study on size of reference set. Here,  \textit{shot} means that how many generated instances per class in synthetic reference set. The bold indicates the best.}\label{table:ablation-reference}
\vspace{-0.2in}\end{table}


==> tables/adapt-lambda.tex <==
\begin{table}[t]
\centering
\hspace*{\fill}
\parbox[t]{0.4\textwidth}{
\centering\small
\caption{\textcolor{blue}{Ablation study on zero-shot adaptation schemes. Bold indicates the best and runner-up is underlined.}
}\label{table:ablation_component}
\vspace{-0.11in}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{}&\multicolumn{2}{c}{Adaptation} & \multicolumn{4}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule(lr){2-3} \cmidrule{4-7}
$\varepsilon$& T2I & CLIP &ImageNet&STL&SUN&Food\\
\cmidrule{1-1}\cmidrule(lr){2-3}\cmidrule{4-7}
\multirow{3}{*}{0.5}&\xmark&\xmark&29.6&55.2&28.3&43.6\\
&\cmark&\xmark&\underline{31.8}&\textbf{66.0}&\underline{30.7}&\underline{43.8}\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{\cmark} & \cellcolor{white}{\cmark} &\textbf{34.2}&\textbf{66.0}&\textbf{32.1}&\textbf{45.7}\\
\cmidrule{1-1}\cmidrule(lr){2-3}\cmidrule{4-7}
\multirow{3}{*}{0.1}&\xmark&\xmark&17.6&27.0&17.3&21.8\\
&\cmark&\xmark&\underline{19.4}&\underline{40.8}&\underline{19.3}&\underline{27.3}\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{\cmark} & 
\cellcolor{white}{\cmark} &\textbf{20.6}&\textbf{41.2}&\textbf{22.5}&\textbf{28.9}\\
\midrule
\end{tabular}}
}
~~~~
\parbox[t]{0.5\textwidth}{
\centering\small
\caption{
Ablation study on $\lambda$ \eqref{eq:final-person-loss}. Bold indicates the best.}\label{table:ablation-lambda}
\vspace{-0.03in}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{}&&&\multicolumn{6}{c}{Certified accuracy at $\varepsilon$ (\%)}\\
\cmidrule{4-9}
$\sigma$&$\lambda$&ACR&0.0&0.25&0.5&0.75&1.0&1.25\\
\cmidrule{1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule{4-9}
&0.0\phantom{0}\phantom{0}&0.270&49.6&39.0&30.0&19.6\\
0.25 &0.001&0.280&50.6&40.2&30.8&20.2&&\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{0.01\phantom{0}}  &\textbf{0.292}&\textbf{52.2}&\textbf{43.0}&\textbf{31.8}&\textbf{21.4}&&\\
&0.1\phantom{0}\phantom{0}&0.290&51.8&42.8&31.2&20.6\\
\midrule
&0.0\phantom{0}\phantom{0}&0.358&38.0&32.6&27.8&22.2&18.0&14.4\\
0.50 &0.001&0.379&40.4&35.0&30.0&24.6&\textbf{20.0}&14.6\\
\rowcolor[HTML]{EFEFEF}{\cellcolor{white}{}} & \cellcolor{white}{0.01\phantom{0}}  &\textbf{0.394}&\textbf{44.0}&\textbf{37.0}&\textbf{30.8}&\textbf{25.2}&19.4&15.2\\
&0.1\phantom{0}\phantom{0}&0.390&43.4&37.0&30.4&24.2&\textbf{20.0}&\textbf{15.4}\\
\bottomrule
\end{tabular}}}
\hspace*{\fill}
\end{table}

==> tables/algorithm-infer.tex <==
\begin{figure}[t]\centering
{\small
\begin{minipage}[t]{\columnwidth}\centering
\begin{algorithm}[H]
\caption{\textsc{Predict} of our framework}
\label{algro:zero-ar}
\begin{spacing}{1.2}
\begin{algorithmic}[1]

\Require Fine-tuned denoised network $\varepsilon_{\theta^*}$ and classifier $f_{\psi^*}$ through zero-shot adapation schemes, The number of  classes $K$.

\algrule

\Function{\textsc{Predict}}{$\sigma, x, n, \alpha$}

\State $\texttt{counts} = \texttt{zeros}(K)$
\For{$i=1$ to $n$}
\State Sample Gaussian noise $\delta$ from $\mathcal{N}(0, \sigma^2 \textbf{I})$
\State $\hat{x} = x + \delta$ \Comment{Noising $x$ by adding $\delta$ to $x$}
\State $\tilde{x} = \mathtt{denoise}_{\theta^*}(\hat{x})$ \Comment{Denoising $\hat{x}$ in Eq.~\eqref{eq:one-step-denoising-super}}
\State $\texttt{idx} = \operatorname{argmax}(f_{\psi^*}(\tilde{x}))$\\ \Comment{predict label with $f_{\psi^*}$}
\State $\texttt{counts}[\texttt{idx}] \mathrel{+}= 1$
\EndFor
\State $\hat{c}_A, \hat{c}_B \leftarrow \text{top two indices in counts}$
\State $n_A, n_B \leftarrow \texttt{counts}[\hat{c}_A], \texttt{counts}[\hat{c}_B]$
\If{$\textsc{BinomPValue}(n_A, n_A + n_B, 0.5)\leq\alpha$}
\State\Return$\hat{c}_A$
\Else
\State\Return\textsc{ABSTAIN}
\EndIf 

\EndFunction
\end{algorithmic}
\end{spacing}
\end{algorithm}
\end{minipage}
}
\end{figure}


==> tables/clean-robust.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\centering\small
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}[-1em]{}&\multicolumn{5}{c}{Sample size $n$}\\
\cmidrule{2-6}
&25&50&100&200&400\\
\midrule
Clean accuracy (\%)&\bf{58.0}&57.0&56.2&55.6&54.2\\
Robust accuracy (\%)&26.0&29.4&31.4&33.0&\bf{35.2}\\
\midrule
\shortstack{Inference time (sec) \\ \scriptsize{} }&\shortstack{\bf{0.64} \\ \scriptsize{$\pm$0.09} } &\shortstack{0.92 \\ \scriptsize{$\pm$0.10} }&\shortstack{1.39 \\ \scriptsize{$\pm$0.08} }&\shortstack{2.56 \\ \scriptsize{$\pm$0.13} }&\shortstack{5.14 \\ \scriptsize{$\pm$0.12} }\\
\bottomrule
\end{tabular}}
\caption{Analysis of clean accuracy \vs robust accuracy at $\varepsilon=1.0$ and per-image inference time on varying $n$ for smoothing. We use a computing cluster with 4 NVIDIA A100 80GB GPUs for this experiment. Bold indicates the best. 
 }\label{table:clean-robust-table}
\end{table}

==> tables/clean_table.tex <==
\begin{table*}[t]
\centering
\caption{\label{clean-table} Comparison of clean accuracy (\%) of the models reported in Table~\ref{table:main-table} on 9 zero-shot classification datasets. 
For smoothed classifiers such as ``CLIP-Smooth'' and ``Ours'', we report empirical clean accuracy. For ``Ours'', we additionally report certified robust accuracy at $\varepsilon=0$ in parentheses, which is often referred as \emph{certified clean accuracy}. Bold indicates the best.
 }\label{table:clean-table}
\vspace{-0.03in}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{clcccccccc|c}
        \toprule
        $\varepsilon$&Method  & STL  & SUN & Cars & Food & Pets & Flower & DTD & Caltech &
         Average \\
        \midrule
        -&CLIP&97.8&56.8&52.7&83.0&85.7&66.3&37.8&81.9&70.3\\
        \midrule
        \multirow{4.5}{*}{0.5}
        &CLIP-Smooth& 75.0 & 46.8 & 42.1 & 52.3 & 66.7 & 43.5 & 17.2 & 68.3 & 51.5 \\
        &Mao et al.,~\cite{mao2023understanding}&\textbf{94.8}&\textbf{60.0}&48.7&69.7&80.8&57.7&34.0&79.7&65.7\\
        \cmidrule{2-11}
        &{\textbf{Ours}} & \bf{94.8} & 58.6 & \bf{54.1} & \bf{80.2} & \bf{83.6} & \bf{61.4} & \bf{42.7} & \bf{81.7} & \bf{69.6} \\
        &\multicolumn{1}{r}{(Certified)} &(90.4) & (55.4) & (49.7)&(74.5) & (81.9)& (58.7)&(38.9)& (79.1)&(66.1) \\
        \midrule
        \multirow{4.5}{*}{1.0}
        &CLIP-Smooth & 32.4 & 27.7 & 40.8 & 31.3 & 43.8 & 36.8 & \phantom{0}7.0 & 54.0 & 34.2 \\
&Mao et al.,~\cite{mao2023understanding}&93.4&58.2&42.9&61.2&77.0&53.6&30.8&78.5&62.0 \\
        \cmidrule{2-11}
        &{\textbf{Ours}} & \bf{93.8} & \bf{59.4} & \bf{52.9} & \bf{78.8} & \bf{83.1} & \bf{58.9} & \bf{39.1} & \bf{81.7} & \bf{68.5} \\
        &\multicolumn{1}{r}{{(Certified)}} & (80.2) & (53.6)& (45.5)&(64.8)&(77.7)&(48.3) &(32.4)&(75.7)&(59.8)\\
        \bottomrule
       \end{tabular}}
    \vspace{0.03in}
\end{table*}

\iffalse
\begin{table*}[t]
\centering\scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{clcccccccccc}
        \toprule
        \multirow{5}{*}{} & &\multicolumn{9}{c}{\textbf{Dataset}}\\
        \cmidrule{3-11}
        $\varepsilon$&\textbf{Method}  & \rot{STL}  &\rot{SUN}& \rot{StanfordCars}& \rot{Food}& \rot{OxfordPet}& \rot{Flower} &
        \rot{DTD}&\rot{EUROSAT}&\rot{Caltech}&
        \rot{\textbf{Average}}\\
        \midrule
        -&CLIP&97.16&57.76&52.14&83.15&85.82&65.64&40.52&38.26&82.04&66.94\\
        \midrule
        \multirow{3}{*}{0.5}
        &CLIP-Smooth&59.2&33.27&23.66&15.25&50.67&26.12&13.23&15.0&56.37&32.53 \\
        &Mao \textit{et al.}\citep{xx}&\textbf{94.8}&\textbf{59.96}&48.7&69.7&80.76&57.7&33.97&25.0&\textbf{79.68}&61.14\\
        \cmidrule{2-12}
        &\textbf{Ours}&90.4& 55.38& \textbf{49.7}&\textbf{74.46} & \textbf{81.9}& \textbf{58.67}&\textbf{38.92}&\textbf{39.0}&79.08&\textbf{63.05}\\
        \midrule
        \multirow{3}{*}{1.0}
        &CLIP-Smooth&22.2&6.18&2.39&1.19&12.95&6.82&6.06&13.4&23.31&10.5\\
        &Mao \textit{et al.} \citep{xx}&\textbf{93.4}&\textbf{58.17}&42.94&61.18&76.95&\textbf{53.61}&30.78&20.4&\textbf{78.49}&57.32 \\
        \cmidrule{2-12}
        &\textbf{Ours}& 80.2 & 53.59& \textbf{45.52}&\textbf{64.75}&\textbf{77.71}&48.34 &\textbf{32.38}&\textbf{37.8}&75.7&\textbf{57.33}\\
        \bottomrule
       \end{tabular}}
    \caption{Clean accuracies. Empirical methods and certified methods both has different robust model under different perturbation bound, $\varepsilon$=0.5 and 1.0. So, we measure clean accuracies each perturbation level. The best accuracies are \textbf{bolded}.}\label{clean-table}
\end{table*}
\fi

==> tables/imagenet_clean_robust_table.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{}& &\multicolumn{2}{c}{$\varepsilon=0.5$}&\multicolumn{2}{c}{$\varepsilon=1.0$}\\
\cmidrule(lr){3-4}\cmidrule{5-6}
Method & 0-shot & Clean & Robust& Clean & Robust\\
\midrule
CLIP & \cmark &\phantom{0}1.4 \phantom{(00.0)} & \phantom{0}0.2 \phantom{(00.0)} & 58.2 \phantom{(00.0)} & 58.2 \phantom{(00.0)}\\
CLIP-Smooth & \cmark & 16.8 \phantom{0}(9.8) & \phantom{0}2.2 \phantom{0}(1.2)&45.2 (25.0) & 35.2 \phantom{0}(3.8)\\
\bf{Ours} & \cmark &\textbf{42.6} (34.2) & \textbf{31.4} (20.6) &\textbf{56.6} (53.4) & \textbf{56.0} (46.0)\\
\midrule
\citet{mao2023understanding} &\xmark& 26.0 \phantom{(00.0)} & 12.3 \phantom{(00.0)} & 51.2 \phantom{(00.0)} & 47.2 \phantom{(00.0)} \\
\citet{carlini2023diffusion} & \xmark & 38.6 (30.2) & 32.4 (19.8) & 54.8 (49.8) & 53.0 (44.2)\\
\bottomrule
\end{tabular}}
\caption{Clean and robust accuracy (\%) on ImageNet at at $\ell_2$ perturbation bound $\varepsilon=0.5$ and $\varepsilon=1.0$. We reports empirical accuracy and parentheses provide certified accuracy. Bold indicates the best over baselines using ``0-shot" for robustification. We remark that our framework achieves the comparable ImageNet clean and robust accuracy, outperforming baselines using ImageNet full-training set. }\label{imagenet-table}
\end{table}

\iffalse
\begin{table}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cc|cccc}
\toprule
\multirow{2}{*}[-1em]{$\varepsilon$}&\multicolumn{5}{c}{\textbf{Method}}\\
\cmidrule{2-6}
&\multicolumn{1}{c}{CLIP}&CLIP-Smooth&Mao \textit{el al.}\citep{xx}&Carlini \textit{el al.}&\textbf{Ours}\\
\midrule
0.5&\multirow{2}{*}{58.20}&45.20 (\underline{25.00})&51.20&54.82 (\underline{49.83})&\textbf{56.60} (\underline{53.40})\\
\cmidrule{3-6}
1.0&&35.20 \phantom{0}(\underline{3.80})&47.20&53.00 (\underline{44.20})&\textbf{56.00} (\underline{46.00})\\
\bottomrule
\end{tabular}}
    \caption{\label{imagenet-clean-table}ImageNet clean accuracies at $\varepsilon=0.5$ and $\varepsilon=1.0$. We measure each empirical accuracy with 100 step PGD attack and certified accuracy are measured accuracy at \textit{radius} after certification. Specifically, $\varepsilon=0.5(1.0)$ is measured by $\sigma=0.25(0.5)$ smoothed classifer.The best accuracies are \textbf{bolded}.}
    \end{table}
\fi


==> tables/inference_time.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\centering\small
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}[-1em]{}&\multicolumn{5}{c}{Sample size $n$}\\
\cmidrule{2-6}
&25&50&100&200&400\\
\midrule
Inference time (ms)&\bf{639.8}&917.5&1391.9&2559.7&5137.7\\
\bottomrule
\end{tabular}}
\caption{Analysis of inference time on varying sample size for smoothing. Bold indicates requiring the least inference time. 
 }\label{table:infer-time-table}
\end{table}

==> tables/main_table.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of empirical (and certified) robust accuracy (\%) on 9 zero-shot classification datasets, assuming $\ell_2$-adversary with $\varepsilon=0.5$ and $\varepsilon=1.0$. We additionally report certified robust accuracy at $\varepsilon$ for ``Ours'' in parentheses. Bold indicates the best.}\label{table:main-table} 
\vspace{-0.03in}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{clcccccccc|c}
\toprule
$\varepsilon$&Method  & STL  & SUN & Cars & Food & Pets & Flower & DTD & Caltech & Average \\
\midrule
\multirow{5}{*}{0.5}&
        CLIP& 10.8 & \phantom{0}1.2 & \phantom{0}0.0 & \phantom{0}1.8 & \phantom{0}2.7 &\phantom{0}0.8 & \phantom{0}2.7 & 12.0 & \phantom{0}4.0 \\
        &CLIP-Smooth& 42.6 & 23.7 & 14.3 &\phantom{0}8.9& 36.4 & 16.6 & 10.2 & 44.8 & 24.7 \\
        &Mao et al.~\cite{mao2023understanding}&59.4&29.9&12.5&32.9&51.2&33.5&18.8&56.2&36.8\\
        \cmidrule{2-11}
        &{\textbf{Ours}} & \textbf{80.4}& \textbf{41.8}  & \textbf{33.2}&\textbf{59.0} & \textbf{68.6}& \textbf{45.2}&\textbf{29.7}&\textbf{71.3}&\textbf{53.7}\\
        & \multicolumn{1}{r}{(Certified)} & (66.0) & (32.1) &(28.4) &(45.7) &(60.8)& (34.9) &(23.0)&(65.1)&(44.5)\\
        \midrule
        \multirow{5}{*}{1.0}&
        CLIP&\phantom{0}2.4&\phantom{0}0.0&\phantom{0}0.0&\phantom{0}0.2 &\phantom{0}0.2 &\phantom{0}0.2&\phantom{0}1.0&\phantom{0}7.8&\phantom{0}1.5 \\
        &CLIP-Smooth&16.2&\phantom{0}5.8& \phantom{0}1.6&\phantom{0}0.4&\phantom{0}6.7&\phantom{0}4.5&\phantom{0}5.4&18.7&\phantom{0}7.4\\
        &Mao et al.~\cite{mao2023understanding}&21.2&11.0&\phantom{0}2.8&10.3&23.2&14.4&12.0&33.9&16.1 \\
        \cmidrule{2-11}
        & {\textbf{Ours}}& \textbf{66.0} & \textbf{38.3}&  \textbf{27.0}&\textbf{47.3}&\textbf{59.6} &\textbf{33.1} &\textbf{24.9}&\textbf{64.1}&\textbf{45.0}\\
        & \multicolumn{1}{r}{(Certified)} &(41.2)& (22.5)  &(18.9) &(28.9) & (46.5)&(18.9)&(18.2)&(55.8)&(31.4)\\
        \bottomrule
\end{tabular}}

\end{table*}

\iffalse
\begin{table*}[t]
\centering\scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{clcccccccccc}
        \toprule
        
        \multirow{5}{*}{} & &\multicolumn{9}{c}{\textbf{Dataset}}\\
        \cmidrule{3-11}
        $\varepsilon$&\textbf{Method}  & \rot{STL}  &\rot{SUN}& \rot{StanfordCars}& \rot{Food}& \rot{OxfordPet}& \rot{Flower} &
        \rot{DTD}&\rot{EUROSAT}&\rot{Caltech}&
        \rot{\textbf{Average}}\\
        \midrule
        \multirow{5.5}{*}{0.5}&
        CLIP& 10.8 & 1.2&0.0 &1.78&2.67&0.78&2.71&0.0&11.95&3.54 \\
        &CLIP-Smooth& 42.6&23.7 &14.3&8.91&36.38&16.57&10.21&13.6&44.82&23.45 \\
        &Mao \textit{et al.}\citep{xx}&59.4&29.88&12.52&32.87&51.24&33.53&18.82&0.6&56.18&32.78\\
        \cmidrule{2-12}
        &\multirow{2}{*}{\textbf{Ours}} & \textbf{80.4}& \textbf{41.83}  & \textbf{33.2}&\textbf{59.0} & \textbf{68.57}& \textbf{45.22}&\textbf{29.66}&\textbf{29.0}&\textbf{71.31}&\textbf{50.91}\\
        && (\underline{66.0}) & (\underline{32.07}) &(\underline{28.43}) &(\underline{45.74}) &(\underline{60.76})& (\underline{34.89}) &(\underline{22.97})&(\underline{11.0})&(\underline{65.13})&(\underline{40.78})\\
        \midrule
        \multirow{5.5}{*}{1.0}&
        CLIP&2.4&0.0 &0.0&0.19 &0.19 &0.19&0.96&0.0&7.77&1.3 \\
        &CLIP-Smooth&16.2&5.78& 1.59&0.4&6.67&4.48&5.42&11.8&18.73&7.9\\
        &Mao \textit{et al.} \citep{xx}&21.2&10.96&2.78&10.3&23.24&14.42&11.96&0.0&33.86&14.3 \\
        \cmidrule{2-12}
        &\multirow{2}{*}{\textbf{Ours}}& \textbf{66.0} & \textbf{38.25}&  \textbf{27.04}&\textbf{47.32}&\textbf{59.62} &\textbf{33.14} &\textbf{24.88}&\textbf{28.2}&\textbf{64.14}&\textbf{43.18}\\ &&(\underline{41.2})& (\underline{22.5})  &(\underline{18.89}) &(\underline{28.91}) & (\underline{46.48})&(\underline{18.91})&(\underline{18.18})&(\underline{5.6})&(\underline{55.78})&(\underline{28.49})\\
        \bottomrule
       \end{tabular}}
       \caption{Zero-shot robust accuracies at $\varepsilon=0.5$ and $\varepsilon=1.0$. We measure each empirical accuracy with 100 step PGD attack and certified accuracy are measured accuracy at \textit{radius} after certification. Specifically, $\varepsilon=0.5(1.0)$ is measured by $\sigma=0.25(0.5)$ smoothed classifer.The best accuracies are \textbf{bolded}.}\label{table:main-table} 
\end{table*}
\fi
